Beyond the Trees: Resilient Multipath for Last-mile WISP Networks

Expanding the reach of the Internet is a topic of widespread interest today. Google and Facebook, among others, have begun investing substantial research efforts toward expanding Internet access at the edge. Compared to data center networks, which are relatively over-engineered, last-mile networks are highly constrained and end up being ultimately responsible for the performance issues that impact the user experience. The most viable and cost-effective approach for providing last-mile connectivity has proved to be Wireless ISPs (WISPs), which rely on point-to-point wireless backhaul infrastructure to provide connectivity using cheap commodity wireless hardware. However, individual WISP network links are known to have poor reliability and the networks as a whole are highly cost constrained. Motivated by these observations, we propose Wireless ISPs with Redundancy (WISPR), which leverages the cost-performance tradeoff inherent in commodity wireless hardware to move toward a greater number of inexpensive links in WISP networks thereby lowering costs. To take advantage of this new path diversity, we introduce a new, general protocol that provides increased performance, reliability, or a combination of the two.

==> discussion.tex <==
\section{Discussion}

Our primary aim in this paper was to make a case for RAIL and showed the potential network cost and/or capacity gains achievable by augmenting WISP topologies. However, we have not explored whether we can identify the \emph{optimal} links to add to a topology. In addition, there remains much work to be done in further designing and implementing RAIL.

==> experiment.tex <==
\section{Experimental Setup}
\label{s:simulation}

\subsection{Implementation}
\subsubsection{OVS}
Flows installed to enable bootstrap and create the control plane. Traffic destined for controller has eth destination modified to be broadcast, and put in a GRE tunnel.

Match flows installed to know when node itself is the RAIL destination, those packets are sent to RAIL daemon process running on the node.

\subsubsection{RAIL network ingress / egress}
Where do we encapsulate regular IP packets with RAIL stuff? Two choices:

\textbf{OVS}. OVS knows all of the paths so it has to be the one that sets the GRE source and dest (RAIL ingress and egress). I've been operating under this assumption, but it might get tricky / slow in reality since GRE tunneling typically happens using routing rules. Somehow we have to encapsulate, then, before the packet leaves the box, modify the outer IP options field to insert the \# of packets and RAIL mode info and pass to the daemon. I don't know SDN stuff well enough to know how well that will play out.

\textbf{Daemon}. If we tried to hand bare packet to the ingress daemon, we somehow have to convey the egress RAIL node IP in order to construct the GRE header. Doesn't seem reasonable to me right now, unless doing the above in OVS is terrible in terms of performance.

\textbf{END:} OVS adds GRE header, daemon modifies the GRE key. Daemon needs to know for a given session (sent to it by OVS or controller): 4 bits for rail mode, some number of bits for num packets in a group. index and bitmask are state kept in the RAIL daemon and do not have to be sent to the daemon by OVS.  


\subsubsection{RAIL daemon}
Don't modify OVS, OVS sends traffic that matches flow rules (i.e. traffic encapsulated in RAIL headers) to our daemon.

\subsubsection{RAIL encapsulation}
We use GRE headers - 32 bits of space in the key field in a GRE header.

4 bits for RAIL mode, 16 bits for bitmask, 12 bits for array index.

\subsubsection{Dedupe}
Hashmaps for each RAIL mode in which duplication may occur (mirroring) with the hashmap key being the session. 

\subsubsection{RAIL state}
Each mode gets a hash table. Each source gets a hash table.

\subsection{Testbed}
Address the requirements we spelled out in HotNets:
\begin{itemize}
	\item Performance-reliability tradeoff.
	\item Latency-free.
	\item Incrementally-deployable.
	\item Low cost.
	\item Backbone-oriented.
	\item Asymmetric.
	\item Adaptive
\end{itemize}
\subsection{Analytical}




\subsection{Lab testbed}


